Shift Graphs, Chromatic Number and Acyclic One-Path Orientations

Shift graphs, which were introduced by Erd\H{o}s and Hajnal, have been used to answer various questions in extremal graph theory. In this paper, we prove two new results using shift graphs and their induced subgraphs. 1. Recently Girao [Combinatorica2023], showed that for every graph $F$ with at least one edge, there is a constant $c_F$ such that there are graphs of arbitrarily large chromatic number and the same clique number as $F$, in which every $F$-free induced subgraph has chromatic number at most $c_F$. We significantly improve the value of the constant $c_F$ for the special case where $F$ is the complete bipartite graph $K_{a,b}$. We show that any $K_{a,b}$-free induced subgraph of the triangle-free shift graph $G_{n,2}$ has chromatic number bounded by $\mathcal{O}(\log(a+b))$. 2. An undirected simple graph $G$ is said to have the AOP Property if it can be acyclically oriented such that there is at most one directed path between any two vertices. We prove that the shift graph $G_{n,2}$ does not have the AOP property for all $n\geq 9$. Despite this, we construct induced subgraphs of shift graph $G_{n,2}$ with an arbitrarily high chromatic number and odd-girth that have the AOP property. Furthermore, we construct graphs with arbitrarily high odd-girth that do not have the AOP Property and also prove the existence of graphs with girth equal to $5$ that do not have the AOP property.

==> misc.tex <==
\begin{theorem} \label{odd girth}
    If $G$ has odd girth equal to $2g-1$, then the odd girth of $S(G)$ is greater than or equal to $2g+1$.
\end{theorem}
\begin{proof}
     Let  $v_1,v_2, \ldots, v_n$ be the ordering $\sigma$ of the vertices of $G$ that is used to construct $S(G)$. Let $\B=\{B_{v_i}, i=1, 2, \ldots , n\}$ be the bag decomposition of $S(G)$.
  

We will go on to create a sequence of cycles $\{C_i\}$, where each $C_i=\{u^i_1, u^i_2, \ldots u^i_{m_i}\}$ would consist of some vertices from $C_{i-1}$ and one vertex obtained by contracting two vertices of $C_{i-1}$. We also define an index function $I$ on the vertices of $C_i$, which assigns each vertex $v \in C_i$ to a natural number $I(v) \leq n$. We will create the sequence in a way so that each cycle $C_i$ of the sequence  satisfies the following conditions:

\begin{itemize}
    \item (Property 1) The cardinality of $C_i$ is always odd.
\item (Property 2) The vertices $v_{I(u^i_1)}, v_{I(u^i_2)}, v_{I(u^i_3)}, \ldots , v_{I(u^i_{m_i})}, v_{I(u^i_1)}$ forms a circuit in $G$.
\item (Property 3) If $I(u^i_p)=I(u^i_q)$ then $u^i_p$ and $u^i_q$ are non-adjacent in $C_i$.

\end{itemize} 

Also we want to the sequence to have the additional property that $|C_i|>|C_{i+1}|$.

Let $C=\{u^1_1, u^1_2, \ldots, u^1_{m_1}\}$ be a odd cycle of $S(G)$ with $m_1 \leq 2g-1$. 
 Let $u^1_j \in B_{v_{p_j}}$ for all $j=1, 2, 3, \ldots , k$. Define an index function $I$ on the vertices of $C_1$ such that $I(u^1_j)=p_j$. Thus for the cycle $C$, the function $I$ indicates which bag of $S(G)$ the vertex $u^1_j$ belongs to. By observation~\ref{structure of S(G)} and by definition of $I$, $C$ satisfies property $2$ and $3$. Since $|C|$ is odd it trivially satisfies property $1$. \\
 So let $C_1=C$ be the first cycle of the sequence we will construct.  
 
We will show that $I(u^1_{j}), j=1, 2, \ldots, m_1$ cannot be all distinct.
 Let $I(u^1_{j^*})= \max(I(u^1_j)), j=1, 2, 3, \ldots m_1$. Let $u^1_{j^*-1}$ and $u^1_{j^*+1}$ be two neighbours of $u^1_{j^*}$ in the cycle $C_1$. Now since $u^1_{j^*}$ is a vertex of $B_{v_{I(u^1_{j^*})}}$ and since $I(u^1_{j^*})$ is maximum, all the neighbours of $u^1_{j^*}$ in $C_1$ must belong to the same bag. Hence $I(u^1_{j^*-1})=I(u^1_{j^*+1})$. So if $C_1$ is a triangle we have a contradiction as the vertices $u^1_{j^*-1}$ and $u^1_{j^*-1}$  are non-adjacent as they belong to the same bag. Now contract the vertices  $u^1_{j^*-1}$ and $u^1_{j^*-1}$ to create a single vertex $u^*$. So by \ref{breaking an odd cycle} there will be an odd cycle containing the newly created vertex $u$. Call that cycle $C_2$.  Set $I(u)=I(u^1_{j^*-1})$ and the value of the function $I$ for the other vertices of the cycle $C_2$, is same as the value of the function $I$ when it was the part of the cycle $C_1$. Clearly $|C_2| \leq 2g-3$. Let $C_2=\{u^2_1=u^*, u^2_2, u^2_3, \ldots, u^2_{m_2}\}$. It is easy to observe that since $C_1$ satisfied properties $1$, $2$ and $3$, the cycle $C_2$ is created in such a way that it also inherits and hence satisfies properties $1$, $2$ and $3$. 

Now if $I(u^2_i)$ are all distinct then by property $2$ of the cycle $C_2$, we have a cycle of size $|C_2| \leq 2g-3$ in $G$ which is a contradiction. Now if  $I(u^2_i)$ are not all distinct and $C_2$ is a triangle then by observation~\ref{structure of S(G)} we have a contradiction. Else we construct $C_3$ by identifying some two vertices $u^2_{j^*-1}$ and $u^2_{j^*-1}$ of $C_2$ such that $I(u^2_{j^*-1})=I(u^2_{j^*+1})$ and contracting them to create a new vertex $u$. Then by observation \ref{breaking an odd cycle} we have an odd cycle in the newly formed graph containing the vertex $u$. We let $C_3$ be this odd cycle with $I(u)=I(u^2_{j^*-1})$ and the value of the function $I$ for the other vertices of the cycle $C_3$ is same as the value of the function $I$ when it was the part of the cycle $C_2$. 

Now if we keep on forming $C_{i+1}$ from $C_i$ in the same way as $C_3$ was formed from $C_2$ then we will eventually get a cycle $C_j$ which is either a triangle or $I(u^j_i)$ are all distinct, both of which gives a contradiction.  
 
 
\end{proof}



\begin{observation} \label{breaking an odd cycle}
   If $C$ is an odd cycle which is not a triangle and $u_1, u_2$ be two non-adjacent vertices of $C$ then the graph formed by contraction of the vertices $u_1$ and $u_2$ into a single vertex $u$ contains an odd cycle containing $u$.
\end{observation}
\begin{proof}
    Trivial.
\end{proof}

\begin{observation} \label{structure of S(G)}
    In the bag decomposition $\B$ of $S(G)$, any two vertices of $S(G)$ belonging to the same bag are never adjacent. Also for any two adjacent vertices $u_1, u_2$ of $S(G)$ with $u_1 \in B_{v_{i_1}}$ and  $u_2 \in B_{v_{i_2}}$ then $v_{i_1}$ and $v_{i_2}$ are adjacent in $G$. 
\end{observation}





In this section, using any mother graph $G$ we construct a completely new graph $S(G)$. Each vertex of $S(G)$ corresponds to a single vertex of $G$, and we choose the neighbours of the vertices of $S(G)$ by using the structure of $G$ and the correspondence of the vertices of $S(G)$ with the vertices of $G$. We call $S(G)$ the shift of the graph $G$ and study various properties of it. Below, we make our construction precise.


\emph{Construction of S(G):} Given a simple undirected graph $G$, let $\{v_1, v_2, v_3, \ldots , v_n\}$ be an ordering $\sigma$ of $V(G)$. For a vertex $v_j \in V(G)$, let $N^*_G(v_j)=\{v_i: 1\leq 
 i<j \; \text{and} \; v_i \; \text{is adjacent to} \; v_j\}$. Let $d^*(v_j)=|N^*_G(v_j)|$. Let $N^*_G(v_j)= \{v_{j_{k}}, 1\leq k \leq d^*(v_j)$\}, with $j_1 < j_2 < j_3 \cdots, j_{d^*(v_j)}<j$. Now we create vertices of $S(G)$ which correspond to $v_j \in G$. Let $B({v_j})$ be a collection of $d^*(v_j)+1$ vertices of $S(G)$ that correspond to the vertex $v_j \in G$. Let the vertices of $B({v_j})$ be $\{u_{j,i}: 1\leq i \leq d^*(v_j)+1\}$.


We now construct the graph $S(G)$ in an online manner in $|V(G)|$ steps with respect to the ordering $\sigma$.
Initially, we have an empty graph. In the $j^{th}$ step:
\begin{itemize}
    \item Add the vertices of $B({v_j})$ as isolated vertices.
\item For each $i<j$ with $v_i$ adjacent to $v_j$ in $G$, choose a unique vertex $u_{j,x}$ of $B({v_j})$  and then add $|B({v_i})|$ edges to make $u_{j,x}$ adjacent to all the vertices of $B({v_i})$.
\end{itemize} 

Observe that for $i_1 \neq i_2< j$ if $v_{i_1}$ and $v_{i_2}$ are adjacent to $v_j$ in $G$ then the chosen vertex in the $j^{th}$ step with respect to $i_1$ is different than that of the chosen vertex with respect to $i_2$. To be more precise, we now fix an index for the choice of $u_{j,x}$ in the $j^{th}$ step. If $i<p$ and $v_i$ is adjacent to $v_p$, then in the $p^{th}$ step of the construction we choose the vertex $u_{p,q}$ to connect to all the vertices of $B(v_i)$ only if $v_{p_q} \in N^*_G(v_p) =v_i$. Now we can define $S(G)$ more concretely. So, it is the graph with the vertex set $V(S(G))= \bigcup\limits_{i=1}^{n} B(v_i)$ and if $i < p$ then $u_{i,j}$ adjacent to $u_{p,q}$ iff $v_{p_q} \in N^*_G(v_p)=v_i$. 

Note that the condition $v_{p_q} \in N^*_G(v_p)=v_i$ implies that $v_{p}$ must be adjacent to $v_{i}$ in $G$.
We call the collection $\B=\{B(v_i): i=1, 2, \ldots , n\}$ the bag decomposition of the graph $S(G)$ with respect to the given ordering $\sigma$. We also call the sets of vertices $B(v_i)$ as the bag of vertices of $S(G)$. We also define $S^g(G)=S(S^{g-1}(G))$, with $g\in \mathbb{N}$ and $S^1(G)=S(G)$ and $S^0(G)=S(G)$. So $S^g(G)$ is the shift of the graph $S^{g-1}(G)$ with respect to some ordering of the vertices of $S^{g-1}(G)$. 

\emph{Remark:} Observe that the graph $S(G)$ very much depends on the initial ordering $\sigma$ of the vertices of $G$, in fact $S_{\sigma}(G)$ might have been a better notation but in this note we will explore properties of $S(G)$ which are ordering independent and hence we take the liberty in choosing the notation. Also similarly, in order to define $S^g(G)$ uniquely, we need to specify what ordering we have for $G$, then we also need to select an ordering on $S(G)$, $S^2(G)$, \ldots $S^{g-1}(G)$, but here we ignore the orderings in the sense that one is free to choose some ordering. We do this because we are going to only prove results which are ordering independent and holds true for any chosen set of orderings. In the remainder of the text, whenever we say $S(G)$ or $S^g(G)$, it is to be assumed that these graphs are with respect to some pre-specified orderings of vertices. Also note that since $d^*(v_i) \leq deg(v_i)$ for all $v_i \in V(G)$, the number of vertices of $S(G)$ is trivially upper bounded by $2E(G)+V(G)$ regardless of the ordering $\sigma$ of $V(G)$. See Fig.~\ref{fig:shift of a graph} for an illustration on how the properties of the graph $S(G)$ can be different depending on the ordering $\sigma$. 


\begin{observation}
    The graph $S(K_n)$ is isomorphic to the shift graph $G_{n+1,2}$. 
\end{observation}
\begin{proof}
   Observe that collection of vertices $B^i=\{(x,y) \in V(G_{n+1,2}): x=i\}$ will correspond to the bag of vertices $B(v_{n+1-i})$ in the bag decomposition of $S(K_n)$. It is easy to verify that if we map the vertex $u_{(i,j)}$ of $S(K_n)$ to the vertex $(n+1-i,n+1-i+j)$ of $G_{n+1,2}$, it defines an isomorphism from $S(K_n)$ to $G_{n+1,2}$.
\end{proof}

\begin{observation}
    For any graph $G=(V,E)$, the graph $S(G)$ is an induced subgraph of the shift graph $S(K_{|V(G)|})$. 
    
    %And for any induced subgraph $H$ of $S(K_n)$ there exists a graph $G$ with $|V(G)|\leq n$, such that $H$ is isomorphic to $S(G)$.
\end{observation}
\begin{proof}
     Let  $v_1,v_2, \ldots, v_n$ be the ordering $\sigma$ of the vertices of $G$ that is used to construct $S(G)$. Let $\B=\{B(v_i): i=1, 2, \ldots , n\}$ be the bag decomposition of $S(G)$. Let $\B'=\{B'(w_i): i=1, 2, \ldots , n\}$ be the bag decomposition of $S(K_{|V(G)|})$. 
     Now we will create the graph $S(G)$ from the shift graph $S(K_{|V(G)|})$ by deleting vertices of $S(K_{|V(G)|})$. For any vertex $u \in S(K_{|V(G)|})$, by property $5$ of observation~\ref{structure of S(G)}, we know that either it is not adjacent to any vertex $u'$ of $S(K_{|V(G)|})$ with $I(u')<I(u)$ or there exists an unique number $i<I(u)$ such that $u$ is adjacent to all the vertices of $B'(w_i)$. In the former case we keep the vertex $u$ and in the latter case we check  if $v_i$ is adjacent to $v_{I(u)}$ in $G$ or not. If $v_i$ is not adjacent to $v_{I(u)}$ then we delete $u$ from the graph $S(K_{|V(G)|})$, else we keep $u$. After doing this for all the vertices of the graph $S(K_{|V(G)|})$, it is trivial to observe that we have the graph $S(G)$. 
     
            % Now let $H$ be a induced subgraph of $S(K_n)$. Let $\B=\{B(v_i): i=1, 2, \ldots , n\}$ be the bag decomposition of $S(K_n)$. Let $B'(v_i)=B(v_i) \cap H$. Some of these sets may be empty and hence we ignore them.  So let the collection $\{B'(v_{i_j}: j=1, 2, \ldots , m$ denote all the non-empty sets of the form $B'(v_i)$ with $i_1< i_2 <i_3 \cdots <i_m$. Define a graph $G$ with vertices $w_i, w_2, \ldots w_m$ such that the vertex $w_p$ is adjacent to the vertex $w_q$ iff there exists a vertex in  $B'(v_{i_p}$ which is adjacent to a vertex in $B'(v_{i_q}$. It is easy to see the graph $S_\sigma(G)$ with $\sigma=\{w_1, w_2, \ldots w_m\}$ is isomorphic to $H$.
         
\end{proof}

In this section we discuss some basic structural properties of shift graph and it's induced subgraph and define some notations and terminology which will be used throughout the paper. The line digraph $L(G)$ of a digraph $G$ has as its vertices the arcs of $G$, and has an edge from $ab \in E(G)$ to
$cd \in E(G)$, just if $b = c$. It is well known that the shift graph $G_{n,2}=L(\overrightarrow{T_n})$ where $\overrightarrow{T_n}$ is a oriented complete graph with on $n$ vertices with a chosen ordering of vertices $\{v_1, v_2, \ldots v_n\}$, such that the edge between $v_i$ and $v_j$ is directed from $v_i$ to $v_j$ iff $i<j$. Now given a graph $G$ with $n$ vertices, add a vertex $v^*$ to $G$ which is adjacent to all the vertices of $G$. Let $G^*=G \cup \{v^*\}$. Let $\sigma=\{v_1,v_2, v_3, \ldots, v_n\}$ be a chosen ordering of vertices of $G$. Let $v_{n+1}=v^*$. Let $\overrightarrow{G^*_{\sigma}}$ be a orientation of $G^*$ such that if there is a edge between the vertices $v_i$ and $v_j$ then the edge is directed from $v_i$ to $v_j$ iff $i<j$. Define $S_{\sigma}(G)=L(\overrightarrow{G^*_{\sigma}})$. Also let $B(i)$ be the set of outgoing arcs of the vertex $v_{n+1-i}$ for all $1 \leq i \leq n$. It is clear from definition of $S_{\sigma}(G)$ that $B(i)$ are vertices of $S_{\sigma}(G)$ which form an independent set. Also the set $B(1)$ has just one vertex of $S_{\sigma}(G)$, namely the outgoing arc from $v_n$ to $v^*$. We call  $\B_{\sigma}=\{B(i): i=1, 2, \ldots , n\}$ to be the bag decomposition of $S_{\sigma}(G)$.


It is known that for $n \in \mathbb{N}$, the shift graph $G_{n+1,2}$ is a graph with vertices being the ordered $2$-tuples $a=(a_{1},a_{2})$ with $1\leq a_1 < a_2 \leq n+1$, where two vertices $a=(a_1,a_2)$ and $b=(b_1,b_2)$ are adjacent if $a_1=b_2$ or $a_2=b_1$. The graphs $S(G)$ have direct connection to the graphs $G_{n,2}$, in the sense that the graph $S(G)$ is an induced subgraph of the shift graph $G_{|V(G)|+1, 2}$. This is noted in the observations below.





\begin{proof}
Let $c'$ be a proper colouring of $S(G)$ with strictly less than $\log_{2}(\chi(G)+1)$ colours. Let $C'$ be the set of all the different colours used in $c'$. Let  $v_1,v_2, \ldots, v_n$ be the ordering $\sigma$ of the vertices of $G$ that is used to construct $S(G)$. Let $\B=\{B(v_i): i=1, 2, \ldots , n\}$ be the bag decomposition of $S(G)$. Let $C^i \subseteq C'$ be the set of distinct colours used by $c'$ to colour the vertices of $B(v_i)$. Let $C=\{c_1,c_2,c_3, \ldots, c_n\}$ be a set of $n$ colours not necessarily distinct such that the colour $c_i$ is the same as the colour $c_j$ iff the set $C^i$ equals $C^j$. Now colour the vertex $v_i$ of the graph $G$ with the colour $c_i$. We will now show that this is a proper colouring of $G$. Let two vertices $v_i$ and $v_j$ are adjacent in $G$. Without loss of generality assume $i<j$, then by property $4$ of observation~\ref{structure of S(G)}, there is a vertex $u^*$ in $B(v_j)$ that is adjacent to all the vertices of $B(v_i)$ in $S(G)$. Now since $c'$ is a proper colouring of $S(G)$, $c'(u^*)$ must be different from the colours in the set $\{c'(u), u \in B(v_i)\}$, hence  $C^j \neq C^i$ which implies $c_j \neq c_i$. Therefore, the colouring of $G$ using colours from $C$ is proper. Also the number of distinct colours in $C$ is equal to the number of distinct sets $C^i$. Now, since each element of $C^i$ is a colour from $C'$ and each $C^i$ is non-empty, so the number of distinct sets $C^i$ is bounded by the total number of subsets of $C'$ minus one. Now, since $|C'| < \log_{2}(\chi(G)+1)$, we have $|C| < 2^{|C'|}-1 <  \chi(G)$, which is a contradiction. Thus, finishing the proof for the lower bound.

    To prove the upper bound we show that if $\chi(G) \leq {k \choose \floor{\frac{k}{2}}}$ then $\chi(S(G)) \leq k$. Observe that any colouring of $G$ with ${k \choose \floor{\frac{k}{2}}}$ colours can be viewed as an assignment of $\floor{\frac{k}{2}}$ subsets of $\{1, 2, \ldots, k\}$ to the vertices of $G$. Our strategy would be to colour the 
\end{proof}

\begin{corollary} \label{chromatic iteration}
    For any $g\in \mathbb{N}$, $\chi(S^g(G)) \geq \log_{2}\log
    _{2}\cdots\log_{2} (\chi(G))$, where the logarithm is taken $g$ times.
\end{corollary}

\begin{proof}
  Using the lower bound in Theorem \ref{chromatic number of S(G)}  iteratively $g$ times we get our result.
\end{proof}

Next we move on to show that the odd girth of $S(G)$ is strictly bigger than the odd girth $G$. We give some standard definitions that are needed for our proof.

A walk $W$ on a graph $G$ is an alternating sequence of vertices $v_1, v_2, \ldots$ and edges $e_1, e_2 \ldots,$ of $G$, beginning and ending with a vertex and each edge $e_j$ of $W$ is incident with the vertex $v_j$ and the vertex $v_{j+1}$. In simple graphs only specifying the vertices is enough as the edges between two vertices are unique. A closed walk is a walk that starts and ends in the same vertex. Also, the length of a walk is the number of edges in it.
 Before we proceed to our theorem, we state a standard lemma below. For the sake of completeness, we give a sketch of the proof.

\begin{lemma} \label{odd cycle}
  In any simple undirected graph $G$, every closed walk with odd length contains an odd cycle.
\end{lemma}
\begin{proof}
    We proceed by induction on the length of the walk. Trivially, in a simple graph, there cannot be an odd walk of length $1$. So we have our base case when the closed walk $v_1, e_1, v_2, e_2, v_3, e_3, v_1$ has length $3$. Clearly, since $G$ is simple, $v_2 \neq v_1$ and $v_3\neq v_2 $ and $v_3\neq v_1$. So all the 3 vertices must be distinct and hence its a odd cycle of length $3$.

Now, let any closed odd walk of length $2g-1$ have an odd cycle. Let $$W=v_1, e_1, v_2, e_2, v_3, e_3, \ldots v_{2g+1}, e_{2g+1}, v_1$$ be a closed walk of length $2g+1$. Now if all the vertices $v_i$, $1 \leq i \leq 2g+1$ are distinct then it is an odd cycle and we are done. Now suppose that $W$ has $2$ repeated vertex (say $v_i=v_j$, $i<j$). Then clearly they cannot be consecutive as $G$ is simple. So we can divide the walk $W$ into two distinct closed walks $W_1$, $W_2$ both starting with $v_i$ and ending in $v_j$ where $W_1=v_i, v_{i+1}, \ldots, v_j$ and $W_2=v_i, v_{i-1}, \ldots , v_1, v_{2g+1}, \ldots, v_j$. Since each of the walks has a size greater than or equal to $2$, each of the walks will have a size less than or equal to $2g-1$, and trivially one of them must be an odd walk. Hence, by induction we are done.
\end{proof}



\begin{theorem} \label{odd girth}
    If $G$ has an odd girth equal to $2g-1$, then the odd girth of $S(G)$ is greater than or equal to $2g+1$.
\end{theorem}
\begin{proof}
     Let  $v_1,v_2, \ldots, v_n$ be the ordering $\sigma$ of the vertices of $G$ that is used to construct $S(G)$. Let $\B=\{B(v_i): i=1, 2, \ldots , n\}$ be the bag decomposition of $S(G)$.
  




Let $C=\{u_1, u_2, \ldots, u_{m}\}$ be an odd cycle of $S(G)$ with $m \leq 2g-1$. 
By the property $2$ of observation~\ref{structure of S(G)}, we know that $W= v_{I(u_1)}, v_{I(u_2)}, v_{I(u_3)}, \ldots , v_{I(u_m)}, v_{I(u_1)}$ forms a closed walk in $G$. We will show that $I(u_{j}), j=1, 2, \ldots, m$ cannot be all distinct.
 Let $I(u_{j^*})= \max_{1 \leq j \leq m}(I(u_j))$, where the maximum is attained for the vertex $u_{j^*} \in S(G)$. Let $u_{j^*_1}$ and $u_{j^*_2}$ be two neighbours of $u_{j^*}$ in the cycle $C$. Now since $I(u_{j^*})$ is maximum among the index values of the vertices in the cycle $C$ so by property $3$ of observation~\ref{structure of S(G)}, we have $I(u_{j^*_1})=I(u_{j^*_2})$. Hence $W$ contains repeated vertices and therefore is not a cycle in $G$. Also by lemma~\ref{odd cycle}, we know that $G$ has an odd cycle consisting of vertices from $W$, so the length of that odd cycle must be strictly less than $2g-1$ which is a contradiction because the odd girth of $G$ is $2g-1$. Hence, no odd cycle of $S(G)$ can have length less than or equal to $2g-1$, so we are done.  
 
\end{proof}


\begin{corollary}\label{girth iteration}
    Given any simple undirected graph $G$, the odd girth of the graph $S^g(G)$ is greater than or equal to $2g+1$.
\end{corollary}

\begin{proof}
Trivially follows from repeated application of Theorem~\ref{odd girth}.

\end{proof}

It is not hard to observe that given any graph $G$, the graph $S(G)$ has many induced $4$-holes, which makes it intuitive to believe that the chromatic number of any $4$-hole-free induced subgraph is small. In the following theorem we verify indeed it is the case, in fact the chromatic number of any $4$-hole-free induced subgraph is bounded by $4$.

\begin{theorem} \label{square free induced}
   For any simple undirected graph $G$ and for natural number $g$, any $4$-hole-free induced subgraph $H$ of $S^g(G)$ satisfies $\chi(H)\leq 4$.
\end{theorem}
\begin{proof}
   Note that it is sufficient to prove that any $4$-hole-free induced subgraph $H$ of $S(G)$ satisfies $\chi(H)\leq 4$.
   Let  $v_1,v_2, \ldots, v_n$ be the ordering $\sigma$ of the vertices of $G$ that is used to construct $S(G)$. Let $\B=\{B(v_i): i=1, 2, \ldots , n\}$ be the bag decomposition of $S(G)$. 

Let $B'({v_i})=B(v_i) \cap H, \; \text{for all} \; i=1, 2, \ldots , n$. Let 
$$L= \bigcup\limits_{v_i:|B'(v_i)|=1} B'(v_i) \; \; \text{and} \; \; R= \bigcup\limits_{v_i: |B'(v_i)| \geq 2} B'(v_i).$$ 

$L$ is the set of all vertices $u\in H$ such that $B(v_{I(u)})$ is a singleton set containing only the vertex $u$. And $R$ is the set of all vertices $u\in H$ such that $B(v_{I(u)})$ has at least one more vertex other than $u$.

Let ${T_L}$ denote the induced subgraph of $H$ on $L$. Similarly let $T_R$ denote the induced subgraph of $H$ on $R$.

\emph{Claim 1: The graph $T_L$ is a tree}\\
Let $C=\{u_1, u_2, \ldots, u_{m}\}$ be a cycle of $T_L$. Let $I(u_{j^*})= \max_{1\leq j \leq m}(I(u_j))$, where the maximum is attained for the vertex $u_{j^*} \in T_L$. Observe for any two vertices $u,u'$ of $T_L$, $I(u) \neq I(u')$. Let $u_{j^*_1}$ and $u_{j^*_2}$ be two neighbours of $u_{j^*}$ in the cycle $C$. Now since $I(u_{j^*})$ is maximum among the index values of the vertices in the cycle $C$ so by property $3$ of observation~\ref{structure of S(G)}, we have $I(u_{j^*-1})=I(u_{j^*+1})$. Hence we have a contradiction. So $T_L$ has no cycles and hence must be a tree.


\emph{Claim 2: The graph $T_R$ is a tree.}

Let $C=\{u_1, u_2, \ldots, u_{m}\}$ be a cycle of $T_R$. Let $I(u_{j^*})= \min_{j \leq 1 \leq m}(I(u_j))$, where the minimum is attained for the vertex $u_{j^*} \in T_R$. Let $u_{j^*_1}$ and $u_{j^*_2}$ be two neighbours of $u_{j^*}$ in the cycle $C$. Since $T_R$ is an induced subgraph of $G$, hence by property $4$ of observation~\ref{structure of S(G)}, $u_{j^*_1}$ and $u_{j^*_2}$ are adjacent to all the vertices of $B'(v_{I(u_{j^*})})$.
Since $B'(v_{I(u_{j^*})})\in R$, it has at least $2$ vertices. So $B'(v_{I(u_{j^*})})\in R$ has at least one more vertex other than $u_{j^*}$, call that vertex as $u'$. So we know that $u_{j^*_1}$ and $u_{j^*_2}$ are adjacent to both $u_{j^*}$ and $u'$ in $T_R$. 

Now by minimality of $I(u_{j^*})$, we have $I(u')=I(u_{j^*})<I(u_{j^*_1})$ and $I(u')=I(u_{j^*})<I(u_{j^*_2})$.
Now suppose that the vertices $u_{j^*_1}$ and $u_{j^*_2}$ are adjacent in $T_R$. So by property $1$ of observation~\ref{structure of S(G)}, we have $I(u_{j^*_1})\neq I(u_{j^*_2})$. So without loss of generality assume $I(u_{j^*_1})<I(u_{j^*_2})$. Hence we have $u_{j^*_2}$ adjacent to $u_{j^*}$ and $u_{j^*_1}$ in $T_R$ with $I(u_{j^*_1})<I(u_{j^*_2})$ and $I(u_{j^*})<I(u_{j^*_2})$. Now since $T_R$ is an induced subgraph, by property $3$ of observation~\ref{structure of S(G)}, we have $I(u_{j^*})=I(u_{j^*_1})$ which by property $1$ of observation~\ref{structure of S(G)}, gives a contradiction. So we know that the vertices $u_{j^*_1}$ and $u_{j^*_2}$ are non-adjacent in $T_R$.  Now again by property $1$ of observation~\ref{structure of S(G)}, we know that the vertices $u_{j^*}$ and $u'$ are non adjacent in $T_R$.   

So the vertices $u_{j^*_1}, u_{j^*}, u_{j^*_2}, u'$ induces a $4$-hole in $T_R$ and hence in $H$, which is a contradiction. Hence the graph $T_R$ does not have any cycle and so must be a tree.

Let $c_1,c_2,c_3,c_4$ be $4$ distinct colours. Since $T_L$ is a tree, we can have a proper colouring of $T_L$ with two colours $c_1$ and $c_2$. Similarly we can have a proper colouring of $T_R$ with two colours $c_3$ and $c_4$. So this gives a colouring of all the vertices of $H$ as $V(H)=V(T_L) \cup V(T_R)$. We show that this is a proper colouring of $H$. Suppose if $u,u'$ are two adjacent vertices in $H$, then if both $u,u'$ are in $T_L$ or in $T_R$, then they get different colours as the colouring of $T_R$ and $T_L$ is proper. Now if $u \in T_L$ and $u' \in T_R$, then they also get different colours as $c_1,c_2,c_3,c_4$ are all distinct. Hence we are done.



\end{proof}







\subsection{Construction of high odd girth and high chromatic graphs with local chromatic number bounded by $3$} \label{subsec:Local Chromatic Number}

Using the construction of the shift of a graph in Section~\ref{construction} and using its properties proved in Section~\ref{subsec:Chromatic number}, in this section we give explicit construction of graphs with high chromatic number, high odd girth and local chromatic number bounded by $3$. 


Let $X_n= \{1, 2, 3, \ldots, n\}$. The shift graph $G_{n,3}$ is the graph formed by the vertex set is the set of all triples $(x_0, x_1, x_2)$ with
$x_0, x_1, x_2 \in X_n$. And if $x_0 <x_1 <x_2$ and $y_0 <y_1 <y_2$, 
$x_1 = y_0$, $x_2 = y_1$, then the vertices $(x_0, x_1, x_2)$ and $(y_0, y_1, y_2)$ are joined. In~\cite{ERDOS198621}, Erdos~\etal proved the following interesting result.

\begin{theorem} \label{Erdos}
~\cite{ERDOS198621} If $n$ goes to infinity then $\chi(G_{n,3})$ goes to infinity and the local chromatic number of $G_{n,3}$ is always bounded by $3$.
\end{theorem}

Now we prove a fairly straightforward lemma showing that the local chromatic number of $S(G)$ is upper bounded by the local chromatic number of $G$. 

\begin{lemma} \label{local chromatic bound}
    The local chromatic number of $S(G)$ is less than or equal to the local chromatic number of $G$.
\end{lemma}

\begin{proof}
    Let $c$ be a proper colouring of $G$ such that the number different colours used by $c$ to colour $N_G(v)$ is at most $k$ for any vertex $v\in G$. We now define a colouring $c'$ of $S(G)$. For any vertex $u\in S(G)$, let $c'(u)=c(v_{I(u)})$.
From the property $2$ of observation~\ref{structure of S(G)}, we know that that if $u$ and $u'$ are adjacent in $S(G)$ then $v_{I(u)}$ and $v_{I(u')}$ are adjacent in $G$. So the colouring $c'$ of $S(G)$ is proper because the colouring $c$ of $G$ is proper. Again from the property $2$ of observation~\ref{structure of S(G)}, the number of colours used by $c'$ to colour $N_{S(G)}(u)$ is exactly equal to the number of colours used by $c$ to colour $N_G(v_{I(u)})$. Hence $c'$ is a proper colouring of $S(G)$ for which the number of colours used in $N_{S(G)}(u)$ is at most $k$ for any vertex $u\in G$. Thus finishing the proof.
\end{proof}

Hence we have the following result.
\begin{theorem}
    Let $g \in \mathbb{N}$ be fixed. Then chromatic number of the sequence of graphs $\{S^g(G_{n,3})\}$ goes to infinity as $n$ goes to infinity and all the graphs in the sequence $\{S^g(G_{n,3})\}$ has odd girth greater than or equal to $2g+3$ and local chromatic number bounded by $3$.
\end{theorem}

\begin{proof}
    From Theorem~\ref{Erdos} and corollary \ref{chromatic iteration}, we have that the chromatic number of the sequence of graphs $\{S^g(G_{n,3})\}$ goes to infinity as $n$ goes to infinity. From corollary \ref{girth iteration}, we know that all the graphs in the sequence $\{S^g(G_{n,3})\}$ has odd girth greater than or equal to $2g+3$ as the graph $G_{n,3}$ has odd girth equal to $5$. And finally from lemma \ref{local chromatic bound}, we have that $\psi(S^g(G_{n,3}) \leq \psi(S^{g-1}(G_{n,3}) \leq  \cdots \leq \psi(S(G_{n,3}) \leq \psi(G_{n,3}) \leq 3$. Thus finishing the proof.
\end{proof}

